Beyond File-Level Splits: Rethinking Symbolic Music Evaluation via Multi-View Alignment

Symbolic music generation often continues MIDI passages by predicting subsequent notes or events. Held-out prediction loss can overestimate generalization to unseen compositions when training contains another performance or arrangement of a test work. We introduce Multi-View Alignment-Aware Same-Work Identification, combining complementary musical representations with temporal alignment of shared passages to remove test-work versions from training while preserving unrelated material and fixing evaluation files. In a controlled cohort of 100 manually verified pairs selected for high embedding similarity, replacing 3.29% of training windows with test-work versions reduces mean per-group NLL by up to 30.16% relative to matched unrelated content. Across two datasets and two generators, our method brings test losses closest to a reference built from independent work labels. Compared with removing the same number of files at random, it leaves fewer test works exposed and retains more eligible content, including about 99% of eligible tokens on the piano-performance dataset. A separate study on that dataset matches training tokens and updates: no test works remain exposed under the dataset labels, and mean relative test loss is 2.15% higher than an independently selected reference. These findings support keeping all versions of each composition in one split when evaluating generalization to unseen works. The project is available at https://kunbai05-nb.github.io/.

==> experiments/tables/generation_metrics.tex <==
% Generated by render_multidimensional_tables.py; do not hand-edit values.
\multicolumn{9}{@{}l}{\textbf{ATEPP}} \\
\cmidrule(lr){1-9}
Uncorrected & $36.09\,{\scriptstyle\pm\,0.78}$ & $59.14\,{\scriptstyle\pm\,0.86}$ & $22.42\,{\scriptstyle\pm\,0.92}$ & $7.49\,{\scriptstyle\pm\,0.07}$ & $39.21\,{\scriptstyle\pm\,0.21}$ & $61.26\,{\scriptstyle\pm\,1.35}$ & $23.89\,{\scriptstyle\pm\,0.71}$ & $6.78\,{\scriptstyle\pm\,0.03}$ \\
Matched random removal & $29.03\,{\scriptstyle\pm\,0.96}$ & $49.76\,{\scriptstyle\pm\,0.91}$ & $10.92\,{\scriptstyle\pm\,0.94}$ & $8.68\,{\scriptstyle\pm\,0.08}$ & $32.27\,{\scriptstyle\pm\,0.31}$ & $52.12\,{\scriptstyle\pm\,1.16}$ & $11.69\,{\scriptstyle\pm\,0.42}$ & $7.87\,{\scriptstyle\pm\,0.01}$ \\
\rowcolor{mvablue!7}
\textbf{MVA-SWI isolation} & $22.49\,{\scriptstyle\pm\,0.65}$ & $40.88\,{\scriptstyle\pm\,1.03}$ & $3.64\,{\scriptstyle\pm\,0.27}$ & $10.14\,{\scriptstyle\pm\,0.07}$ & $25.53\,{\scriptstyle\pm\,0.64}$ & $43.05\,{\scriptstyle\pm\,1.24}$ & $4.06\,{\scriptstyle\pm\,0.46}$ & $9.13\,{\scriptstyle\pm\,0.07}$ \\
CAugBERT $\cup$ CLaMP & $19.02\,{\scriptstyle\pm\,1.00}$ & $36.60\,{\scriptstyle\pm\,0.42}$ & $2.28\,{\scriptstyle\pm\,0.10}$ & $11.04\,{\scriptstyle\pm\,0.06}$ & $22.21\,{\scriptstyle\pm\,0.45}$ & $39.07\,{\scriptstyle\pm\,0.86}$ & $3.03\,{\scriptstyle\pm\,0.29}$ & $9.96\,{\scriptstyle\pm\,0.07}$ \\
\emph{Label-isolated reference} & $22.05\,{\scriptstyle\pm\,1.04}$ & $40.80\,{\scriptstyle\pm\,0.95}$ & $3.33\,{\scriptstyle\pm\,0.17}$ & $10.02\,{\scriptstyle\pm\,0.08}$ & $25.29\,{\scriptstyle\pm\,0.48}$ & $43.35\,{\scriptstyle\pm\,1.24}$ & $3.94\,{\scriptstyle\pm\,0.43}$ & $9.06\,{\scriptstyle\pm\,0.07}$ \\
\addlinespace[4pt]
\multicolumn{9}{@{}l}{\textbf{LMD-clean}} \\
\cmidrule(lr){1-9}
Uncorrected & $33.80\,{\scriptstyle\pm\,1.81}$ & $55.66\,{\scriptstyle\pm\,0.39}$ & $21.90\,{\scriptstyle\pm\,1.86}$ & $9.00\,{\scriptstyle\pm\,0.08}$ & $37.58\,{\scriptstyle\pm\,1.11}$ & $60.40\,{\scriptstyle\pm\,1.31}$ & $22.30\,{\scriptstyle\pm\,1.40}$ & $8.31\,{\scriptstyle\pm\,0.02}$ \\
Matched random removal & $26.75\,{\scriptstyle\pm\,1.71}$ & $46.87\,{\scriptstyle\pm\,0.03}$ & $10.48\,{\scriptstyle\pm\,1.37}$ & $10.45\,{\scriptstyle\pm\,0.07}$ & $30.70\,{\scriptstyle\pm\,0.95}$ & $51.61\,{\scriptstyle\pm\,1.51}$ & $11.01\,{\scriptstyle\pm\,0.22}$ & $9.65\,{\scriptstyle\pm\,0.01}$ \\
\rowcolor{mvablue!7}
\textbf{MVA-SWI isolation} & $19.71\,{\scriptstyle\pm\,1.79}$ & $37.33\,{\scriptstyle\pm\,0.10}$ & $2.46\,{\scriptstyle\pm\,0.56}$ & $12.15\,{\scriptstyle\pm\,0.11}$ & $23.87\,{\scriptstyle\pm\,1.00}$ & $42.58\,{\scriptstyle\pm\,1.16}$ & $3.33\,{\scriptstyle\pm\,0.78}$ & $11.24\,{\scriptstyle\pm\,0.01}$ \\
CAugBERT $\cup$ CLaMP & $16.53\,{\scriptstyle\pm\,2.10}$ & $33.53\,{\scriptstyle\pm\,0.14}$ & $1.29\,{\scriptstyle\pm\,0.26}$ & $13.18\,{\scriptstyle\pm\,0.12}$ & $20.80\,{\scriptstyle\pm\,0.82}$ & $38.36\,{\scriptstyle\pm\,1.00}$ & $2.13\,{\scriptstyle\pm\,0.70}$ & $12.21\,{\scriptstyle\pm\,0.02}$ \\
\emph{Label-isolated reference} & $19.69\,{\scriptstyle\pm\,1.65}$ & $37.67\,{\scriptstyle\pm\,0.29}$ & $2.41\,{\scriptstyle\pm\,0.49}$ & $11.97\,{\scriptstyle\pm\,0.12}$ & $23.64\,{\scriptstyle\pm\,0.95}$ & $42.83\,{\scriptstyle\pm\,1.30}$ & $3.22\,{\scriptstyle\pm\,0.90}$ & $11.11\,{\scriptstyle\pm\,0.02}$ \\

